H-SemiS: Hierarchical Fusion of Semi and Self-Supervised Learning for Knee Osteoarthritis Severity Grading

Knee osteoarthritis (KOA) is a degenerative joint disease that can lead to chronic pain, reduced mobility, and long-term disability. Automated severity grading from knee radiographs can support early assessment, but current methods heavily depend on large labeled datasets and remain sensitive to class imbalance, noisy samples, and variability in clinical annotations. To alleviate these limitations, we propose a Hierarchical fusion of Semi-Supervised framework with Self-Supervision (H-SemiS) for KOA severity grading in knee X-ray samples using limited annotated data. Rather than treating severity grading as a flat multi-class problem, H-SemiS decomposes the task into a sequence of binary sub-tasks within a semi-supervised teacher-student architecture, directly mitigating the impact of class imbalance. To further enhance feature learning from unlabeled data, the framework integrates an adversarial self-supervised reconstruction module that encourages the network to capture robust anatomical structures. In parallel, a teacher-student design with quantum-inspired feature mixing improves discrimination boundaries between adjacent grades when pseudo-labels are noisy. We comprehensively evaluate H-SemiS on two challenging multi-class datasets and assess its generalizability on two binary-class datasets. Our experimental results demonstrate the superiority of the proposed H-SemiS framework across multiple evaluation metrics, consistently outperforming several competing baselines and state-of-the-art methods. The code is publicly available at https://github.com/chandravardhan-singh-raghaw/H-SemiS.

==> tikzlibrarysecdia.code.tex <==
% = = = = = = = = = = = = = = = = 
% Sector diagram library 7/10/2013
% = = = = = = = = = = = = = = = = 
%\usepackage{pgfplots}
\usetikzlibrary{backgrounds,calc,shapes.geometric}
\pgfdeclarelayer{sector-back}
\pgfdeclarelayer{sector-middle}
\pgfsetlayers{sector-back,sector-middle,main}

\newcommand{\deflistentries}[1]{
\gdef\listentries{}% global list
\foreach \x[count=\xi] in {#1}{\global\let\maxitems\xi}% count the max number of items
\foreach \x[count=\xi] in {#1}{
 \ifnum\xi=\maxitems
   \xdef\listentries{\listentries \x}
 \else
   \xdef\listentries{\listentries \x,}
 \fi  
}
}
\newcommand{\deflistcolors}[1]{
\gdef\listcolors{}% global list
\foreach \x[count=\xi] in {#1}{\global\let\maxitemcolors\xi}% count the max number of items
\foreach \x[count=\xi] in {#1}{
 \ifnum\xi=\maxitemcolors
   \xdef\listcolors{\listcolors \x}
 \else
   \xdef\listcolors{\listcolors \x,}
 \fi  
}
}

% list of keys
\pgfkeys{/tikz/.cd,
  diagram angle/.store in=\refangle,
  diagram angle=30,
  diagram radius/.store in=\diagramradius,
  diagram radius=5,
  diagram step/.store in=\diagramstep,
  diagram step=1,
  diagram axes precision/.store in=\diagramprecision,
  diagram axes precision=0,
  diagram x label/.store in=\diagramxlabel,
  % diagram x label=Test A,
  diagram x label=,
  diagram y label/.store in=\diagramylabel,
  % diagram y label=Test B,
  diagram y label=,
  diagram x label pos/.store in=\diagramxlabelpos,
  diagram x label pos=135:\diagramradius,
  diagram y label pos/.store in=\diagramylabelpos,
  diagram y label pos=270:\diagramradius,
  options x label/.store in=\diagramxoptions,
  options x label={},
  options y label/.store in=\diagramyoptions,
  options y label={},
  draw axes/.code={
    \pgfmathsetmacro\diagramsecondstep{2*\diagramstep}
    \begin{pgfonlayer}{sector-back}
    \foreach \angle in {0,\refangle,...,360}{
      \draw[help lines,dashed](0,0) --++(\angle:\diagramradius);
    }
    \draw(-\diagramradius,0)--(\diagramradius,0);
    \draw(0,-\diagramradius)--(0,\diagramradius);
    \foreach \x in {\diagramstep,\diagramsecondstep,...,\diagramradius}{
      \draw[help lines,dashed](0,0) circle[radius=\x];
      \draw(\x,0.1)--(\x,-0.1);
      \draw(0.1,\x)--(-0.1,\x);
      \draw(-\x,0.1)--(-\x,-0.1);
      \draw(0.1,-\x)--(-0.1,-\x);
    }
    \end{pgfonlayer}

     \foreach \x in {\diagramstep,\diagramsecondstep,...,\diagramradius}{ 
      \node[fill=white,draw,inner sep=1.5pt,font=\footnotesize] at (0,\x)
      {\pgfmathprintnumber[fixed,
        precision=\diagramprecision,
        fixed zerofill,
      ]{\x}};
    }
    \node[fill=white,draw,inner sep=1.5pt] at (0,0){0};
    \node[fill=white,\diagramxoptions] at (\diagramxlabelpos){\diagramxlabel};
    \node[fill=white,\diagramyoptions] at (\diagramylabelpos){\diagramylabel};
  },
  sector angle/.store in=\sectorangle,
  sector angle=\refangle,
  sector color/.store in=\sectorcolor,
  sector color=green!80!black,
  sector opacity/.store in=\sectoropacity,
  sector opacity=0.8,
  sector amplitude/.store in=\sectoramplitude,
  sector amplitude=1cm,
  sector rotation/.store in=\sectorrotation,
  sector rotation=\sectorangle/2,
  sector amplitude=1,
  draw sector/.code={
    \begin{pgfonlayer}{sector-middle}
    \node[circular sector,
          draw,
          fill=\sectorcolor,
          opacity=\sectoropacity,
          circular sector angle=\sectorangle,
          anchor=sector center,
          minimum width=\sectoramplitude,
          rotate=\sectorrotation] 
          at (0,0){};
    \end{pgfonlayer}
  },
  draw sector list/.code={
    \foreach \ampli/\thiscolor[count=\xi from 0] in {#1}{
            \pgfmathtruncatemacro\thisrotation{\sectorangle/2+\xi*\sectorangle}
            \sector[sector color=\thiscolor,
               sector amplitude=\ampli,
               sector rotation=\thisrotation,
               draw sector]{};
    }
  },
}

\tikzset{sector legend/.style={
  circular sector,
  draw,
  opacity=\sectoropacity
  }
}
% definition to insert numbers
\pgfkeys{/pgfplots/sector in legend/.style={%
        /pgfplots/legend image code/.code={%
            \node[sector legend,#1] at (0,0){}; 
        },%
    },
}

% main commands
\def\drawaxes{\tikz@path@overlay{node}}
\def\sector{\tikz@path@overlay{node}}
\def\sectorlist{\tikz@path@overlay{node}}
\def\sectorlegendimage#1{\addlegendimage{sector in legend={#1}}}
\def\legendlistcolors#1{%
\pgfplotsinvokeforeach{#1}{
\sectorlegendimage{fill=##1}}
}

% legend stuff
%%--------------------------------
% Code from Christian Feuersänger
% https://tex.stackexchange.com/questions/54794/using-a-pgfplots-style-legend-in-a-plain-old-tikzpicture#54834

% argument #1: any options
\newenvironment{customlegend}[1][]{%
    \begingroup
    % inits/clears the lists (which might be populated from previous
    % axes):
    \csname pgfplots@init@cleared@structures\endcsname
    \pgfplotsset{#1}%
}{%
    % draws the legend:
    \csname pgfplots@createlegend\endcsname
    \endgroup
}%

% makes \addlegendimage available (typically only available within an
% axis environment):
\def\addlegendimage{\csname pgfplots@addlegendimage\endcsname}

%%--------------------------------
